Consumption Factor Optimization for Multihop Relaying over Nakagami-m Fading channels

In this paper, the energy efficiency of multihop relaying over Nakagami-$m$ fading channels is investigated. The "consumption factor" is used as a metric to evaluate the energy efficiency, and it is derived in closed-form for both amplify-and-forward and decode-and-forward relaying. Then, based on the obtained expressions, we propose a power allocation strategy maximizing the consumption factor. In addition, two sub-optimal, low complexity, power allocation algorithms are proposed and analyzed, and the obtained power allocation schemes are compared, in terms of energy efficiency as well as other common performance metrics, to other power allocation schemes from the literature. Analytical and simulation results confirm the accuracy of our derivations, and assess the performance gains of the proposed approach.

==> Biblio_IEEE_TVT.tex <==
Automatically generated by Mendeley Desktop 1.11
Any changes to this file will be lost if it is regenerated by Mendeley.

BibTeX export options can be customized via Options -> BibTeX in Mendeley Desktop



@ARTICLE{Murdock2014,
author={Murdock, J.N. and Rappaport, T.S.},
journal={Selected Areas in Communications, IEEE Journal on},
title={Consumption Factor and Power-Efficiency Factor: A Theory for Evaluating the Energy Efficiency of Cascaded Communication Systems},
year={2014},
month={February},
volume={32},
number={2},
pages={221-236},
keywords={energy conservation;energy consumption;radio networks;radio receivers;radio transmitters;telecommunication power supplies;Shannon's fundamental limit theory;cascaded circuits;cascaded communication systems;cascaded components;consumption factor theory;energy consumption;energy efficiency;energy efficient architectures;energy efficient design choices;error-free communication;general communication system;green engineering;network architectures;power consumption;power-efficiency factor;propagation path loss;relay transmitter;source transmitter;wireless communication networks;wireless link;Capacity;Cascaded circuits;Energy Efficiency;Millimeter-wave;Power Consumption;Power Efficiency;Relay channel;Wireless},
doi={10.1109/JSAC.2014.141204},
ISSN={0733-8716},}



@book{gradshteyn2007,
  added-at = {2011-05-02T05:41:34.000+0200},
  author = {Gradshteyn, I. S. and Ryzhik, I. M.},
  biburl = {http://www.bibsonomy.org/bibtex/2bae535b4ef6bc86a7a04e6de6fa4d311/peter.ralph},
  description = {MR: Publications results for "MR Number=(2360010)"},
  edition = {Seventh},
  interhash = {1850c3bd20bb756bfc17136ec16a9a7c},
  intrahash = {bae535b4ef6bc86a7a04e6de6fa4d311},
  isbn = {978-0-12-373637-6; 0-12-373637-4},
  keywords = {reference},
  mrclass = {00A22 (33-00 65-00 65A05)},
  mrnumber = {2360010 (2008g:00005)},
  note = {Translated from the Russian, Translation edited and with a preface by Alan Jeffrey and Daniel Zwillinger, With one CD-ROM (Windows, Macintosh and UNIX)},
  pages = {xlviii+1171},
  publisher = {Elsevier/Academic Press, Amsterdam},
  timestamp = {2011-05-02T05:41:34.000+0200},
  title = {Table of integrals, series, and products},
  year = 2007
}

@ARTICLE{Randrianantenaina2014,
author={Randrianantenaina,I. and  Benjillali,M. and  Alouini, M.-S.},
journal={Conference on Communications and Networking , IEEE},
title={Transmit  Power  Optimization for Green Multihop Relaying over  {N}akagami-$m$  Fading  Channels},
year={2014},
month={March},
}






@ARTICLE{Hasna2003,
author={Hasna, M.O. and Alouini, M.-S.},
journal={Communications Letters, IEEE},
title={Outage probability of multihop transmission over Nakagami fading channels},
year={2003},
month={May},
volume={7},
number={5},
pages={216-218},
keywords={fading channels;radio networks;telecommunication network reliability;Laplace transform;Nakagami fading channels;closed-form expression;end-to-end outage probability;end-to-end signal-to-noise ratio;moment generating function;multihop transmission;outage probability;performance;relay gain;wireless communication systems;Closed-form solution;Fading;Frame relay;Laplace equations;Performance gain;Probability;Signal generators;Signal to noise ratio;Spread spectrum communication;Wireless communication},
doi={10.1109/LCOMM.2003.812178},
ISSN={1089-7798},}

